Systematic comparison of semi-supervised and self-supervised learning for medical image classification

In typical medical image classification problems, labeled data is scarce while unlabeled data is more available. Semi-supervised learning and self-supervised learning are two different research directions that can improve accuracy by learning from extra unlabeled data. Recent methods from both directions have reported significant gains on traditional benchmarks. Yet past benchmarks do not focus on medical tasks and rarely compare self- and semi- methods together on an equal footing. Furthermore, past benchmarks often handle hyperparameter tuning suboptimally. First, they may not tune hyperparameters at all, leading to underfitting. Second, when tuning does occur, it often unrealistically uses a labeled validation set that is much larger than the training set. Therefore currently published rankings might not always corroborate with their practical utility This study contributes a systematic evaluation of self- and semi- methods with a unified experimental protocol intended to guide a practitioner with scarce overall labeled data and a limited compute budget. We answer two key questions: Can hyperparameter tuning be effective with realistic-sized validation sets? If so, when all methods are tuned well, which self- or semi-supervised methods achieve the best accuracy? Our study compares 13 representative semi- and self-supervised methods to strong labeled-set-only baselines on 4 medical datasets. From 20000+ GPU hours of computation, we provide valuable best practices to resource-constrained practitioners: hyperparameter tuning is effective, and the semi-supervised method known as MixMatch delivers the most reliable gains across 4 datasets.

==> App_related_work.tex <==
%% integrated with App B



==> Makefile <==
## To build paper PDF: 'make main.pdf'

SHELL=/bin/bash

MAIN?=cvpr_main

TEX_FILES_EXCEPT_MAIN=$$(bash -c "find . -name '*.tex' -maxdepth 1 | sort -n | grep -v ${MAIN}.tex")
TMP_RESULT=$$(bash -c "find . -name '*.tex' -maxdepth 1 | xargs grep "figures/" | cut -d':' -f2 | grep -v '%'");
PDF_FIG_FILES=$$(python -c "print(' '.join([s + ('.pdf' * (1 - s.endswith('.pdf')) * (1 - s.endswith('.png'))) for s in [x.partition('}')[0] for x in '''${TMP_RESULT}'''.split('{')] if s.startswith('figures/')]))")
PNG_FIG_FILES=$$(python -c "print(' '.join([s for s in [x.partition('}')[0] for x in '''${TMP_RESULT}'''.split('{')] if s.startswith('figures/') and s.endswith('.png') ]))")
JPG_FIG_FILES=$$(python -c "print(' '.join([s for s in [x.partition('}')[0] for x in '''${TMP_RESULT}'''.split('{')] if s.startswith('figures/') and s.endswith('.jpg') ]))")

OUTPUTFILE_DOCX?=$(MAIN).docx
BIBLIO_OPTS = --bibliography *.bib --csl apa.csl

all: $(MAIN).pdf $(MAIN).docx

clean:
	rm -fv *.zip *.aux *.log *.bbl *.blg *.ptc *.toc *.out *.lot *.lof *.dvi *.ps *.pdf *.docx

clean_extras:
	rm -fv *.aux *.bbl *.blg *.toc *.out *.lot *.lof

pdf: $(MAIN).pdf

paper: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).bbl *.tex
	# Run 3x to get cross refs right
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) && rm -fv *.aux *.blg *.toc *.out *.lot *.lof

$(MAIN).bbl: $(MAIN).tex *.tex *.bib
	pdflatex -interaction nonstopmode $(MAIN) || true
	bibtex $(MAIN) && rm $(MAIN).pdf

main_to_submit.pdf: main.pdf
	gs -sDEVICE=pdfwrite -dNOPAUSE -dBATCH -dSAFER -dFirstPage=1 -dLastPage=14 -sOutputFile=main_to_submit.pdf main.pdf

$(OUTPUTFILE_DOCX): *.tex *.bib figures/*.pdf
	pandoc $(MAIN).tex \
		--from latex \
		--to docx \
		--output $(OUTPUTFILE_DOCX) \
		$(BIBLIO_OPTS)

src_for_arxiv.zip: $(MAIN).bbl $(MAIN).tex *.tex *.bib
	zip -r src_for_arxiv.zip \
		*.bbl \
		$(MAIN).tex \
		$(TEX_FILES_EXCEPT_MAIN) \
		$(PDF_FIG_FILES) \
		$(PNG_FIG_FILES) \
		$(JPG_FIG_FILES)


==> _packages_to_import.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{microtype}      % microtypography
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{enumitem}

%% Table of contents (needs to come before hyperref!)
\usepackage{titletoc}
\usepackage[page,header]{appendix}

%% Hyperlinks
\usepackage[hyphens]{url}            % simple URL typesetting
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    citecolor=blue,
    filecolor=blue,
    linkcolor=blue,
    urlcolor=blue,
}

%% Figures
\usepackage{graphicx}
\usepackage{chngcntr} % make figure numbering in appendix work
% Suppress weird warnings about pdf page groups
\begingroup
	\expandafter\ifx\csname pdfsuppresswarningpagegroup\endcsname\relax\else\global\pdfsuppresswarningpagegroup=1\relax\fi
\endgroup

%% Tables
\usepackage{tabularx}
\usepackage{wrapfig}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{tablefootnote}
\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\usepackage{tikz}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}

%%% Math typesetting
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage{scalerel}
\usepackage{bm}

%% Small captions
\usepackage{caption}
\usepackage{subcaption}
\captionsetup[table]{font=small,labelfont=small}
\captionsetup[figure]{font=small,labelfont=small}
%\captionsetup[wrapfig]{font=small,labelfont=small}
%\captionsetup[wraptable]{font=small,labelfont=small}

%% Algorithms
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}

%%% SPACE-REDUCING HACK 1/3
% Reduce spacing around section headers
\usepackage{titlesec}
\titlespacing\section{0pt}{0pt plus 2pt minus 0pt}{-2pt plus 2pt minus 0pt}
\titlespacing\subsection{0pt}{0pt plus 2pt minus 0pt}{-2pt plus 2pt minus 0pt}

%%% SPACE-REDUCING HACK 2/3
% Reduce spacing around floats 
\setlength{\floatsep}{8pt plus 4pt minus 4pt}
\setlength{\textfloatsep}{8pt plus 4pt minus 3pt}



==> checklist.tex <==
\section*{Checklist}
\label{sec:checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Limitations paragraph in Sec. 7}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Broader Impacts paragraph in Sec. 7}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See URL on bottom of page one}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See appendix B and C}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, see Fig 2 in main paper. We omitted error bars in Fig 1 and Tab. 3 to reduce clutter, but further results with error bars for the final best checkpoint can be found in App. A}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See appendix}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited all 3 datasets we used in Sec 4.}
  \item Did you mention the license of the assets?
    \answerYes{Yes all are meant for open-access by researchers.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Code is shared at the provided URL}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We clarified that all data is completely de-identified.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> figsrc_acc-over-time-airogs-resnet50.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{CVPR_figures/AIROGS/res50/AIROGS_RAW_TEST_Bacc_unified.pdf}
    \caption{Test accuracy over time on AIROGS with ResNet50.}
    \label{fig:resnet50}
    \vspace{-5mm}
\end{figure}

==> figsrc_valtestgap.tex <==
\begin{figure}[!t]
\setlength{\tabcolsep}{.5mm}
    \begin{tabular}{c c}
%        \includegraphics[width=.23\textwidth]{figures/Variance/TissueMNIST_RAW_unified_4h.pdf}
%    &
%        \includegraphics[width=.23\textwidth]{figures/Variance/TissueMNIST_RAW_unified_50h.pdf}
%    &
%        \includegraphics[width=.23\textwidth]{figures/Variance/TMED_RAW_unified_8h.pdf}
%    &
%        \includegraphics[width=.23\textwidth]{figures/Variance/TMED_RAW_unified_100h.pdf}
%    \\
%    Tissue{\small MNIST} after 4h & Tissue{\small MNIST} after 50h & TMED-2 after 8h & TMED-2 after 100h
%    \\
%        \includegraphics[width=.23\textwidth]{figures/Variance/PathMNIST_RAW_unified_2h.pdf}
%    &
%        \includegraphics[width=.23\textwidth]{figures/Variance/PathMNIST_RAW_unified_25h.pdf}
%    &
        \includegraphics[width=.46\textwidth]{figures/Variance/TMED_RAW_unified_8h.pdf}
    &
        \includegraphics[width=.46\textwidth]{figures/Variance/TMED_RAW_unified_100h.pdf}
    \\
    TMED-2 after 8h & TMED-2 after 100h (full budget)
    \\
        \includegraphics[width=.46\textwidth]{figures/Variance/PathMNIST_RAW_unified_2h.pdf}
    &
        \includegraphics[width=.46\textwidth]{figures/Variance/PathMNIST_RAW_unified_25h.pdf}
    \\ PathMNIST after 2h & PathMNIST after 25h (full budget)
    \end{tabular}
%\vspace{-3mm} % HACK REDUCE WHITESPACE
\caption{
\textbf{Performance variation across independent trials over time.}
Intervals visualize the lowest and highest balanced accuracy of 5 separate trials of Alg.~\ref{alg:hyperparam_tuning}. 
Y-axis shows balanced accuracy. X-axis from left to right shows CoMatch, FlexMatch, FixMatch, MixMatch, Mean-Teacher, Pseudo-labeling, SwAV, MoCo, SimCLR, BYOL and SimSiam. %
More results in Appendix~\ref{app:results}.
%than semi-supervised methods.
}%endcaption
\label{fig:valtestgap}
\end{figure}





% \begin{figure}[!t]
% \setlength{\tabcolsep}{.5mm}
%     \begin{tabular}{c c c c c}
% %        \includegraphics[width=.23\textwidth]{figures/Variance/TissueMNIST_RAW_unified_4h.pdf}
% %    &
% %        \includegraphics[width=.23\textwidth]{figures/Variance/TissueMNIST_RAW_unified_50h.pdf}
% %    &
% %        \includegraphics[width=.23\textwidth]{figures/Variance/TMED_RAW_unified_8h.pdf}
% %    &
% %        \includegraphics[width=.23\textwidth]{figures/Variance/TMED_RAW_unified_100h.pdf}
% %    \\
% %    Tissue{\small MNIST} after 4h & Tissue{\small MNIST} after 50h & TMED-2 after 8h & TMED-2 after 100h
% %    \\
% %        \includegraphics[width=.23\textwidth]{figures/Variance/PathMNIST_RAW_unified_2h.pdf}
% %    &
% %        \includegraphics[width=.23\textwidth]{figures/Variance/PathMNIST_RAW_unified_25h.pdf}
% %    &
%         \includegraphics[width=.28\textwidth]{figures/Variance/TMED_RAW_unified_8h.pdf}
%     &
%         \includegraphics[width=.28\textwidth]{figures/Variance/TMED_RAW_unified_100h.pdf}
%     &
%         \includegraphics[width=.28\textwidth]{figures/Variance/PathMNIST_RAW_unified_25h.pdf}
%     &
% \multicolumn{2}{c}{
% \raisebox{\height}{%HACK fix vertical alignment
% \begin{minipage}{.4\textwidth}
% \begin{small}
% \setlength{\tabcolsep}{.5mm}
% \begin{tabular}{|l r r r r|}\hline
%     & \multicolumn{3}{c}{Acc(val) - Acc(test)} &
%     \\
%  & Tissue & Path  & TMED  &\\ 
% \hline
% Semi & 8.25 & 11.22 & 4.33 & \\ 
% \hline
% Self & 6.88 & -0.06 & 3.86 &\\ 
% \hline
% \end{tabular}
% \end{small}
% \end{minipage}
% }}
%     \\
%     TMED-2 after 8h & TMED-2 after 100h & Path after 25h
%     \end{tabular}
% \vspace{-3mm} % HACK REDUCE WHITESPACE
% \caption{
% \emph{Left 3 panels:}
% \textbf{Performance variation across independent trials over time.}
% Intervals visualize the lowest and highest balanced accuracy of 5 separate trials of Alg. Y-axis showing balanced accuracy. X-axis from left to right showing CoMatch, FlexMatch, FixMatch, MixMatch, Mean-Teacher, Pseudo-labeling, SwAV, MoCo, SimCLR, BYOL and SimS iam~\ref{alg:hyperparam_tuning}.
% More results in Appendix~\ref{app:results}.
% \emph{Right:}
% \textbf{Generalization gap on each dataset} (closer-to-zero indicates more reliability), after the maximum alotted time.
% Self-supervised methods in aggregate appear to have a lower validation-test gap (less risk of overfitting).
% %than semi-supervised methods.
% }%endcaption
% \label{fig:valtestgap}
% \end{figure}

==> tab_valtestconsistency.tex <==
\begin{wraptable}[10]{r}{0.4\textwidth}
\begin{small}
\setlength{\tabcolsep}{.5mm}
\begin{tabular}{|l r r r r|}\hline
    & \multicolumn{3}{c}{Acc(val) - Acc(test)} &
    \\
 & Tissue & Path  & TMED  &\\ 
\hline
Semi & 8.25 & 11.22 & 4.33 & \\ 
\hline
Self & 6.88 & -0.06 & 3.86 &\\ 
\hline
\end{tabular}
\end{small}
\caption{
\textbf{Generalization gap on each dataset} (closer-to-zero indicates more reliability), after the maximum alotted time.
Self-supervised methods in aggregate appear to have a lower validation-test gap (less risk of overfitting).
}
\end{wraptable}
